Temperatures of dust and gas in S~140

In dense parts of interstellar clouds (> 10^5 cm^-3), dust & gas are expected to be in thermal equilibrium, being coupled via collisions. However, previous studies have shown that the temperatures of the dust & gas may remain decoupled even at higher densities. We study in detail the temperatures of dust & gas in the photon-dominated region S 140, especially around the deeply embedded infrared sources IRS 1-3 and at the ionization front. We derive the dust temperature and column density by combining Herschel PACS continuum observations with SOFIA observations at 37 $\mu$m and SCUBA at 450 $\mu$m. We model these observations using greybody fits and the DUSTY radiative transfer code. For the gas part we use RADEX to model the CO 1-0, CO 2-1, 13CO 1-0 and C18O 1-0 emission lines mapped with the IRAM-30m over a 4' field. Around IRS 1-3, we use HIFI observations of single-points and cuts in CO 9-8, 13CO 10-9 and C18O 9-8 to constrain the amount of warm gas, using the best fitting dust model derived with DUSTY as input to the non-local radiative transfer model RATRAN. We find that the gas temperature around the infrared sources varies between 35 and 55K and that the gas is systematically warmer than the dust by ~5-15K despite the high gas density. In addition we observe an increase of the gas temperature from 30-35K in the surrounding up to 40-45K towards the ionization front, most likely due to the UV radiation from the external star. Furthermore, detailed models of the temperature structure close to IRS 1 show that the gas is warmer and/or denser than what we model. Finally, modelling of the dust emission from the sub-mm peak SMM 1 constrains its luminosity to a few ~10^2 Lo. We conclude that the gas heating in the S 140 region is very efficient even at high densities, most likely due to the deep UV penetration from the embedded sources in a clumpy medium and/or oblique shocks.

==> aa.clsV6.0 <==
% This is aa.cls
% A&A DOCUMENT CLASS -- version 6.1 for LaTeX2e
%
% LaTeX document class for Astronomy and Astrophysics journal
%
%%
%%
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesClass{aa}[2006/06/01 v6.1
^^JLaTeX document class for Astronomy and Astrophysics journal]
\newcommand\@ptsize{}
\newif\if@restonecol
\newif\if@titlepage
\@titlepagefalse
\newif\if@longauth
\@longauthfalse
\newif\if@online
\@onlinefalse
\newif\if@rnote
\@rnotefalse
\newif\if@oldversion
\@oldversionfalse
\newif\if@letter
\@letterfalse

%
\DeclareOption{a4paper}
   {\setlength\paperheight {297mm}% 
    \setlength\paperwidth  {210mm}}
\DeclareOption{letterpaper}
   {\setlength\paperheight {11in}%
    \setlength\paperwidth  {8.5in}}
\DeclareOption{legalpaper}
   {\setlength\paperheight {14in}%
    \setlength\paperwidth  {8.5in}}
\DeclareOption{10pt}{\renewcommand\@ptsize{0}}
\DeclareOption{11pt}{\renewcommand\@ptsize{1}}
\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
\DeclareOption{twoside}{\@twosidetrue  \@mparswitchtrue}
\DeclareOption{draft}{\setlength\overfullrule{5pt}}
\DeclareOption{final}{\setlength\overfullrule{0pt}}
\DeclareOption{twocolumn}{\@twocolumntrue}
\DeclareOption{leqno}{\input{leqno.clo}}
\DeclareOption{fleqn}{\input{fleqn.clo}}
\DeclareOption{openbib}{%
  \AtEndOfPackage{%
   \renewcommand\@openbib@code{%
      \advance\leftmargin\bibindent
      \itemindent -\bibindent
      \listparindent \itemindent
      \parsep \z@
      }%
   \renewcommand\newblock{\par}}%
}
%
\DeclareOption{longauth}{\@longauthtrue}
\DeclareOption{rnote}{\@rnotetrue}
\DeclareOption{oldversion}{\@oldversiontrue}
%% January 2008 - abstract
\DeclareOption{traditabstract}{\@oldversiontrue}
\DeclareOption{structabstract}{\@oldversionfalse}
\DeclareOption{letter}{\@lettertrue}
%
\let\if@runhead\iffalse
\DeclareOption{runningheads}{\let\if@runhead\iftrue}
\let\if@envcntreset\iffalse
\DeclareOption{envcountreset}{\let\if@envcntreset\iftrue}
\let\if@envcntsect\iffalse
\DeclareOption{envcountsect}{\let\if@envcntsect\iftrue}
\let\if@referee\iffalse
\DeclareOption{referee}{\let\if@referee\iftrue}
\let\if@onecolumn\iffalse
\DeclareOption{onecolumn}{\let\if@onecolumn\iftrue}
\let\if@nyobjects\iffalse
%
\ExecuteOptions{a4paper,twoside,twocolumn,fleqn,final,10pt,runningheads}
\ProcessOptions
\AtEndOfClass{\mathindent\z@}
%
\if\@ptsize 0
%
   \renewcommand\normalsize{%
      \@setfontsize\normalsize\@xpt{11}%
      \abovedisplayskip 8.55\p@ \@plus4\p@ \@minus5\p@
      \abovedisplayshortskip \z@ \@plus3\p@
      \belowdisplayshortskip 6\p@ \@plus3\p@ \@minus3\p@
      \belowdisplayskip \abovedisplayskip
      \let\@listi\@listI}
   \normalsize
   \newcommand\small{%
      \@setfontsize\small\@ixpt{10}%
      \abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
      \abovedisplayshortskip \z@ \@plus2\p@
      \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
      \def\@listi{\leftmargin\leftmargini
                  \parsep 0\p@ \@plus1\p@ \@minus\p@
                  \topsep 8\p@ \@plus2\p@ \@minus4\p@
                  \itemsep0\p@}%
      \belowdisplayskip \abovedisplayskip
   }
   \newcommand\scriptsize{\@setfontsize\scriptsize\@viipt\@viiipt}
   \newcommand\tiny{\@setfontsize\tiny\@viiipt\@ixpt} 
   \newcommand\large{\@setfontsize\large\@xipt{13}}
   \newcommand\Large{\@setfontsize\Large\@xivpt{16}}
   \newcommand\LARGE{\@setfontsize\LARGE\@xviipt{20}}
   \newcommand\huge{\@setfontsize\huge\@xxpt{24}}
   \newcommand\Huge{\@setfontsize\Huge\@xxvpt{30}}
   %
   \setlength\parindent{15\p@}
   \setlength\smallskipamount{3\p@ \@plus 1\p@ \@minus 1\p@}
   \setlength\medskipamount{6\p@ \@plus 2\p@ \@minus 2\p@}
   \setlength\bigskipamount{12\p@ \@plus 4\p@ \@minus 4\p@}
   \setlength\headheight{12\p@}
   \setlength\headsep   {12\p@} % 
   \setlength\topskip   {10\p@}
   \setlength\footskip{30\p@}
   \setlength\maxdepth{.5\topskip}
   %
   \@settopoint\textwidth
   \setlength\marginparsep {10\p@}
   \setlength\marginparpush{5\p@}
   \setlength\oddsidemargin   {-30\p@}
   \setlength\evensidemargin  {-30\p@}
   \setlength\marginparwidth  {48\p@}
   \setlength\topmargin{-40pt}
   \setlength\footnotesep{8\p@}
   \setlength{\skip\footins}{9\p@ \@plus 4\p@ \@minus 2\p@}
   \setlength\floatsep    {12\p@ \@plus 2\p@ \@minus 2\p@}
   \setlength\textfloatsep{18\p@ \@plus 8\p@ \@minus 6\p@}
   \setlength\intextsep   {18\p@ \@plus 2\p@ \@minus 2\p@}
   \setlength\dblfloatsep    {12\p@ \@plus 2\p@ \@minus 2\p@}
   \setlength\dbltextfloatsep{18\p@ \@plus 8\p@ \@minus 6\p@}
   \setlength\@fptop{0\p@ }
   \setlength\@fpsep{12\p@ }
   \setlength\@fpbot{0\p@ \@plus 1fil}
   \setlength\@dblfptop{0\p@ }
   \setlength\@dblfpsep{12\p@ }
   \setlength\@dblfpbot{0\p@ \@plus 1fil}
   \setlength\partopsep{2\p@ \@plus 1\p@ \@minus 1\p@}
   \def\@listi{\leftmargin\leftmargini
               \parsep \z@
               \topsep 8\p@ \@plus2\p@ \@minus4\p@
               \itemsep\parsep}
   \let\@listI\@listi
   \@listi
   \def\@listii {\leftmargin\leftmarginii
                 \labelwidth\leftmarginii
                 \advance\labelwidth-\labelsep
                 \topsep    \z@
                 \parsep    \topsep
                 \itemsep   \parsep}
   \def\@listiii{\leftmargin\leftmarginiii
                 \labelwidth\leftmarginiii
                 \advance\labelwidth-\labelsep
                 \topsep    \z@
                 \parsep    \topsep
                 \itemsep   \parsep}
   \def\@listiv {\leftmargin\leftmarginiv
                 \labelwidth\leftmarginiv
                 \advance\labelwidth-\labelsep}
   \def\@listv  {\leftmargin\leftmarginv
                 \labelwidth\leftmarginv
                 \advance\labelwidth-\labelsep}
   \def\@listvi {\leftmargin\leftmarginvi
                 \labelwidth\leftmarginvi
                 \advance\labelwidth-\labelsep}
\else
   \input{size1\@ptsize.clo}
\fi
%
\let\footnotesize\small
%
\setlength{\textwidth}{184mm}
\setlength{\textheight}{705pt} 
%
\setlength\lineskip{1\p@}
\setlength\normallineskip{1\p@}
\renewcommand\baselinestretch{}
\setlength\parskip{0\p@ \@plus \p@}
\@lowpenalty   51
\@medpenalty  151
\@highpenalty 301
%
\setcounter{topnumber}{4}
\renewcommand\topfraction{.9}
\setcounter{bottomnumber}{2}
\renewcommand\bottomfraction{.5}
\setcounter{totalnumber}{6}
\renewcommand\textfraction{.05}
\renewcommand\floatpagefraction{.95}
\setcounter{dbltopnumber}{3}
\renewcommand\dbltopfraction{.9}
\renewcommand\dblfloatpagefraction{.95}
%
\def\ps@headings{%
    \let\@oddfoot\@empty\let\@evenfoot\@empty
    \def\@evenhead{\small\rlap{\thepage}\hfil\leftmark\hfil}%
    \def\@oddhead{\small\hfil\rightmark\hfil\llap{\thepage}}%
    \let\@mkboth\@gobbletwo
    \let\sectionmark\@gobble
    \let\subsectionmark\@gobble
    }
% make indentations changeable
\def\setitemindent#1{\settowidth{\labelwidth}{#1}%
        \leftmargini\labelwidth
        \advance\leftmargini\labelsep
   \def\@listi{\leftmargin\leftmargini
        \labelwidth\leftmargini\advance\labelwidth by -\labelsep
        \parsep=\parskip
        \topsep=\medskipamount
        \itemsep=\parskip \advance\itemsep by -\parsep}}
\def\setitemitemindent#1{\settowidth{\labelwidth}{#1}%
        \leftmarginii\labelwidth
        \advance\leftmarginii\labelsep
\def\@listii{\leftmargin\leftmarginii
        \labelwidth\leftmarginii\advance\labelwidth by -\labelsep
        \parsep=\parskip
        \topsep=\z@
        \itemsep=\parskip \advance\itemsep by -\parsep}}
% labels of description
\def\descriptionlabel#1{\hspace\labelsep #1\hfil}
% adjusted environment "description"
% if an optional parameter (at the first two levels of lists)
% is present, its width is considered to be the widest mark
% throughout the current list.
\def\description{\@ifnextchar[{\@describe}{\list{}{\labelwidth\z@
          \itemindent-\leftmargin \let\makelabel\descriptionlabel}}}
\let\enddescription\endlist
%
\def\describelabel#1{#1\hfil}
\def\@describe[#1]{\relax\ifnum\@listdepth=0
\setitemindent{#1}\else\ifnum\@listdepth=1
\setitemitemindent{#1}\fi\fi
\list{--}{\let\makelabel\describelabel}}
%
\newdimen\logodepth
\logodepth=1.3cm
\newdimen\headerboxheight
\headerboxheight=143pt
\newdimen\betweenumberspace          % dimension for space between
\betweenumberspace=3.33pt            % number and text of titles.
\newdimen\aftertext                  % dimension for space after
\aftertext=5pt                       % text of title.
\newdimen\headlineindent             % dimension for space between
\headlineindent=1.166cm              % number and text of headings.
\def\andname{and}
\def\keywordname{Key words.}
\def\lastandname{, and}
\def\mailname{{\it Correspondence to\/}:}
\def\email#1{{e-mail: \tt#1}}
% Used only by the publisher
\def\AASection#1{}
%
\newcounter{inst}
\newcounter{auth}
\newdimen\instindent
\newbox\authrun
\newtoks\authorrunning
\newbox\titrun
\newtoks\titlerunning

\def\journalname#1{\gdef\@journalname{#1}}
\gdef\@journalname{Astronomy \&\ Astrophysics}

\def\headnote#1{\gdef\@headnote{#1}}
\def\@headnote{}

\def\dedication#1{\gdef\@dedic{#1}}
\def\@dedic{}

\let\@date\undefined

\if@oldversion
\long\def\abstract#1{\gdef\@abstract{#1}}
\else
\long\def\abstract#1#2#3#4#5{\gdef\@abstract{\number@fw@rds=0%
         \if!#1!\advance\number@fw@rds-1 \else{\sffamily\itshape Context.}\ \pickupw@rd#1\\\let\WC@go\relax\fi
         {\sffamily\itshape Aims.}\
         \if!#2! \@latex@error{The second heading "Aims" is mandatory in the abstract}{}
           {\it The second heading "Aims" is mandatory in the abstract}\\
           \else\advance\number@fw@rds+1\pickupw@rd#2\\\let\WC@go\relax\fi
         {\sffamily\itshape Methods.}\
         \if!#3! \@latex@error{The third heading "Methods" is mandatory in the abstract}{}
           {\it The third heading "Methods" is mandatory in the abstract}\\
           \else\advance\number@fw@rds+1\pickupw@rd#3\\\let\WC@go\relax\fi
         {\sffamily\itshape Results.}\
         \if!#4! \@latex@error{The forth heading "Results" is mandatory in the abstract}{}
           {\it The forth heading "Results" is mandatory in the abstract}\\
            \else\advance\number@fw@rds+1\pickupw@rd#4\let\WC@go\relax\fi
         \if!#5! \else\\\advance\number@fw@rds+1{\sffamily\itshape Conclusions.}\ \pickupw@rd#5\let\WC@go\relax\fi
         \ifnum\number@fw@rds>400
         \@latex@error{Around \number\number@fw@rds\space words in the abstract instead of 300}{}
         \else\relax\fi}}
\fi

\def\keywords#1{\gdef\@keywords{#1}}
%% January 2007
\def\topics#1{\gdef\@topics{#1}}
\def\@topics{}


\def\institute#1{\gdef\@institute{#1}}

\def\institutename{\par
 \begingroup
 \parindent=0pt
 \parskip=0pt
 \setcounter{inst}{1}%
 \def\and{\par\stepcounter{inst}%
 \hangindent\instindent
 \noindent
 \hbox to\instindent{\hss$^{\theinst}$\enspace}\ignorespaces}%
 \setbox0=\vbox{\def\thanks##1{}\@institute}
 \ifnum\value{inst}>9\relax\setbox0=\hbox{$^{88}$\enspace}%
                 \else\setbox0=\hbox{$^{8}$\enspace}\fi
 \instindent=\wd0\relax
 \ifnum\value{inst}=1\relax
 \else
   \setcounter{inst}{1}%
   \hangindent\instindent
   \noindent
   \hbox to\instindent{\hss$^{\theinst}$\enspace}\ignorespaces
 \fi
 \small
 \ignorespaces
 \@institute\par
 \endgroup}

\def\offprints#1{\begingroup
\def\protect{\noexpand\protect\noexpand}\xdef\@thanks{\@thanks
\protect\footnotetext[0]{\unskip\hskip-1.5em{\it Send offprint requests
to\/}: \ignorespaces#1}}\endgroup\ignorespaces}

\def\mail#1{\gdef\@mail{#1}}
\def\@mail{}

\def\@thanks{}

\def\@fnsymbol#1{\ifcase#1\or\star\or{\star\star}\or{\star\star\star}%
   \or \dagger\or \ddagger\or
   \mathchar "278\or \mathchar "27B\or \|\or **\or \dagger\dagger
   \or \ddagger\ddagger \else\@ctrerr\fi\relax}

\def\inst#1{\unskip$^{#1}$}
\def\fnmsep{\unskip$^,$}

\def\subtitle#1{\gdef\@subtitle{#1}}
\def\@subtitle{}

\def\msnr#1{\gdef\@msnr{#1}}
\def\@msnr{}

\def\idline#1#2{\gdef\@idline{#1}\setcounter{page}{#2}}
\def\@idline{}
\def\doi#1{\gdef\@doi{DOI: 10.1051/0004-6361:#1}}
\def\@doi{(DOI: will be inserted by hand later)}

\def\headnote#1{\gdef\@headnote{#1}}
\def\@headnote{}

\def\ch@ckobl#1#2{\@ifundefined{@#1}
 {\typeout{A\string&A warning: Missing
\expandafter\string\csname#1\endcsname}%
  \csname #1\endcsname{#2}}
 {}}

\def\ch@ckoblabs#1#2#3#4#5#6{\@ifundefined{@#1}
 {\typeout{A\string&A warning: Missing
\expandafter\string\csname#1\endcsname}%
  \csname #1\endcsname{#2}{#3}{#4}{#5}{#6}}
 {}}

\newif\if@normhead \@normheadtrue
\def\hugehead{\@normheadfalse
\onecolumn
\let\thanks=\footnote
\long\def\@makefntext##1{\parindent\bibindent
     \columnwidth\textwidth\advance\columnwidth -\columnsep
     \divide\columnwidth\tw@\hsize\columnwidth \linewidth\columnwidth
     \noindent\hbox to\parindent{\hss$\m@th^{\@thefnmark}$ }##1}%
}

\newcommand\errorref{\@latex@error{Citations are not allowed in the abstract}{}}
\newenvironment{stopref}{\let\cite\errorref\let\citet\errorref\let\citep\errorref}{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This counts the words. This is an extract of  "gvol.sty,
% written by Ivan Andrus (gvol@math.byu.edu)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
  \newcount\number@fw@rds
  \long\def\pickupw@rd#1 {%
    \let\WC@go\pickupw@rd #1
    \advance\number@fw@rds+1
    \expandafter\WC@go
   }
% End of wordcount section

\def\maketitle{\par
\ch@ckobl{journalname}{Noname}
\ch@ckobl{date}{Preprint online version: \today}
\ch@ckobl{title}{A title should be given}
\ch@ckobl{author}{Name(s) and initial(s) of author(s) should be given}
\ch@ckobl{institute}{Address(es) of author(s) should be given}
\if@oldversion
\ch@ckobl{abstract}{An abstract should be given}
\else
\ch@ckoblabs{abstract}{An abstract should be given}{An abstract should be given}
{An abstract should be given}{An abstract should be given}{An abstract should be given}
\fi
\ch@ckobl{keywords}{Keywords should be given}
\begingroup
    \begin{stopref}
    \renewcommand\thefootnote{\@fnsymbol\c@footnote}%
    \def\@makefnmark{$^{\@thefnmark}$}%
 \def\lastand{\ifnum\value{inst}=2\relax
                 \unskip{} \andname\
              \else
                 \unskip, \andname\
              \fi}%
 \def\and{\stepcounter{auth}\relax
          \ifnum\value{auth}=\value{inst}%
             \lastand
          \else
             \unskip,
          \fi}%
 \ifnum \col@number=\@ne
   \@maketitle
 \else
   \twocolumn[\@maketitle]%
 \fi
 \thispagestyle{empty}
 \global\@topnum\z@
 \if@normhead
    \@thanks
 \else
    \twocolumn[\vspace{\@tempdima}]
    \addtocounter{page}{-1}
    \if!\the\authorrunning!
       \authorrunning{ }%
    \fi
 \fi
 \if!\@mail!\else
    \footnotetext[0]{\kern-\bibindent\mailname\
    \ignorespaces\@mail}%
 \fi
%
 \if@runhead
    \def\\{\unskip\ \ignorespaces}\def\inst##1{\unskip{}}%
    \def\thanks##1{\unskip{}}\def\fnmsep{\unskip}%
    \def\object##1{##1}%
    \instindent=\textwidth
    \advance\instindent by-2\headlineindent
    \if!\the\titlerunning!\else
      \edef\@title{\the\titlerunning}%
    \fi
    \global\setbox\titrun=\hbox{\small\rm\unboldmath\ignorespaces\@title}%
    \ifdim\wd\titrun>\instindent
       \typeout{^^JA\string&A Warning: Title too long for running head.}%
       \typeout{Please supply a shorter form with \string\titlerunning
                \space prior to \string\maketitle}%
       \global\setbox\titrun=\hbox{\small\rm
       Title Suppressed Due to Excessive Length}%
    \fi
    \xdef\@title{\copy\titrun}%
%
    \if!\the\authorrunning!
    \else
      \setcounter{auth}{1}%
      \edef\@author{\the\authorrunning}%
    \fi
    \ifnum\value{auth}>2
       \def\stripauthor##1\and##2\endauthor{%
       \protected@xdef\@author{##1\unskip\unskip\if!##2!\else
       \ et al.\fi}}%
       \expandafter\stripauthor\@author\and\endauthor
    \else
       \gdef\and{\unskip\ and \ignorespaces}%
       {\def\and{\noexpand\protect\noexpand\and}%
       \protected@xdef\@author{\@author}}
    \fi
    \global\setbox\authrun=\hbox{\small\unboldmath\@author\unskip:
                                 \unhbox\titrun\if@rnote~\itshape\rnotname\fi}%
    \ifdim\wd\authrun>\instindent
    \typeout{^^JA\string&A Warning: The running head built automatically
             from \string\author\space and \string\title
             ^^Jexceeds the pagewidth, please supply a shorter form
             ^^Jwith \string\authorrunning\space and/or
             \string\titlerunning\space prior to \string\maketitle}%
    \global\setbox\authrun=\hbox{\small\rm Please give a shorter version
       with: {\tt\string\authorrunning\space}and/or{\tt\space
       \string\titilerunning\space}prior to{\tt\space\string\maketitle}}%
    \fi
    \xdef\@author{\copy\authrun}%
    \markboth{\@author}{\@author}%
 \fi
%
 \end{stopref}
 \endgroup
 \setcounter{footnote}{0}
 \setcounter{footnote}{0}%
 \global\let\thanks\relax
 \global\let\maketitle\relax
 \global\let\@maketitle\relax
 \global\let\@thanks\@empty
 \global\let\@author\@empty
 \global\let\@date\@empty
 \global\let\@title\@empty
 \global\let\@subtitle\@empty
 \global\let\@abstract\@empty
%%January 2007
 \global\let\@topics\@empty
 \global\let\@keywords\@empty
 \global\let\keywords\relax
 \global\let\title\relax
 \global\let\author\relax
 \global\let\abstract\relax
 \global\let\date\relax
 \global\let\and\relax}

\def\AALogo{\setbox254=\hbox{
\setlength{\tabcolsep}{0pt}
\begin{tabular}{l}
\\[-30pt]
{\fontsize{18}{21}\selectfont\sffamily\bfseries Astronomy} \\[-2.5pt]
{\fontsize{16}{12}\selectfont\sffamily\mdseries \kern8pt\&\raisebox{4pt}{\rule{78pt}{1pt}}} \\[-5pt]
{\fontsize{18}{21}\selectfont\sffamily\bfseries Astrophysics}
\end{tabular}}\copy254}

\def\makeheadbox{{
\hbox to\textwidth{%
\if!\@idline!
\hbox to0pt{\vbox{\hsize=40cc
\baselineskip=12pt\hrule\hbox
{\vrule\kern3pt\vbox{\kern3pt
\hb@xt@ 40cc{{\sl\@journalname}\ manuscript no.~\jobname \hfill\copyright~ESO~\the\year}
\if!\@msnr!\hbox{\today}\else
\hb@xt@ 30cc{\hfil\strut\LARGE\bfseries\smash{\@msnr}}\fi
\kern3pt}\hfil\kern3pt\vrule}\hrule}\hss}\hfill
\else
\vbox{\baselineskip=11pt
\hbox{\@idline}
\hbox{\@doi}
\hbox{\small\rm \copyright~ESO~\the\year}}
\hfill\AALogo
\fi}}}

\def\@maketitle{\newpage
 \normalfont
 \vbox to0pt{\vskip-20pt
 \nointerlineskip
 \makeheadbox\vss}\nointerlineskip
 \if@normhead
    \setbox\authrun=\vbox\bgroup
 \fi
%% January 2007
 \if!\@topics!\vskip32pt\else
 \vskip24pt
 {\fontsize{12}{14}\selectfont\sffamily {\itshape \@topics} \hfill \fontsize{17}{20}\selectfont\sffamily Special feature}
 \vskip12pt
 \fi
 \begin{center}
%% Januray 2007
%% \vskip24pt
 \if@letter{\large \lettername}\fi
 {\LARGE \sffamily\bfseries\boldmath
  \hrule\@height\logodepth\@width\z@
  \pretolerance=10000
  \vspace*{-12pt}
  \pretolerance=10000
 \if!\@headnote!\else
   \noindent
   {\normalfont\itshape\ignorespaces\@headnote\par}\vskip 3.5mm
 \fi
  \noindent\ignorespaces
  \@title
  \if@rnote \\ \itshape \rnotename \fi
  \par}
 \vskip 8pt\relax
 \if!\@subtitle!\else
   {\Large \sffamily\bfseries\boldmath
   \pretolerance=10000
   \noindent\ignorespaces\@subtitle \par}\vskip 10pt
 \fi
%% \lineskip .5em
 \setbox0=\vbox{\setcounter{auth}{1}\def\and{\stepcounter{auth} }%
                \hfuzz=2\textwidth\def\thanks##1{}\@author}%
 \value{inst}=\value{auth}%
 \setcounter{auth}{1}%
 {\large \rmfamily\mdseries \noindent\ignorespaces\@author}
 \if@longauth \else \end{center} \fi
 \vskip6pt
\small\rm
 \if@longauth {\it (Affiliations can be found after the references)}  \else
 \leftskip=.8cm\rightskip=\leftskip
 \institutename\fi
 \vskip 8pt \noindent\@date
 \if!\@dedic!\else
    \par
    \normalsize\it
    \addvspace\baselineskip
    \noindent\@dedic
 \fi
 \if@longauth \end{center} \fi
 \vskip 8pt
 \small\rm
 \if!\@abstract!\else
  \begin{center}
   {\sffamily\bfseries\abstractname}\par
  \end{center}
  \@abstract
 \fi
 \vskip 6pt
 \small\rm
 \if!\@keywords!\else
 \noindent{\sffamily\bfseries\keywordname}\ \@keywords
 \fi
%
 \if@normhead
    \egroup % end of header box
    \@tempdima=\headerboxheight
    \advance\@tempdima by-\ht\authrun
%   \advance\@tempdima by-\pagetotal
    \ifdim\@tempdima>0pt
       \vrule width0pt height\@tempdima
    \fi
    \unvbox\authrun
    \global\@minipagetrue
    \global\everypar{\global\@minipagefalse\global\everypar{}}
 \else
    \typeout{\the\c@auth\space author names and}
    \typeout{\the\c@inst\space institutes processed}
    \global\@tempdima=\pagetotal
    \global\advance\@tempdima by24pt
 \fi
 \vskip24pt
}
%
\DeclareMathAlphabet{\mathsc}{OT1}{cmr}{m}{sc}
\def\testbx{bx}%
\DeclareRobustCommand{\ion}[2]{%
\relax\ifmmode
\ifx\testbx\f@series
{\mathbf{#1\,\mathsc{#2}}}\else
{\mathrm{#1\,\mathsc{#2}}}\fi
\else\textup{#1\,{\mdseries\textsc{#2}}}%
\fi}
%
\def\clearelargs{\def\1{}\def\2{}\def\3{}\def\4{}\count255=0}
\def\druck@lement#1{{}^{\2}_{\3}\mathrm{#1}{}^{\1}_{\4}{}\if@tempswa$\fi}
\DeclareRobustCommand{\element}{\relax\ifmmode\@tempswafalse
\else$\@tempswatrue\fi\clearelargs\def\?{\phantom{0}}\@lement}
\def\@lement#1{\if#1[\expandafter\f@@dargs\else\druck@lement{#1}\fi}
\def\f@@dargs#1]{\advance\count255by\@ne
\expandafter\def\csname\number\count255\endcsname{#1}\@lement}
%
%\def\vec#1{\ensuremath{\mathbf{#1}}}
\def\vec#1{\ensuremath{\mathchoice{\mbox{\boldmath$\displaystyle#1$}}
{\mbox{\boldmath$\textstyle#1$}}
{\mbox{\boldmath$\scriptstyle#1$}}
{\mbox{\boldmath$\scriptscriptstyle#1$}}}}
%
\def\tens#1{\ensuremath{\mathsf{#1}}}
%
\setcounter{secnumdepth}{3}
\newcounter {section}
\newcounter {subsection}[section]
\newcounter {subsubsection}[subsection]
\newcounter {paragraph}[subsubsection]
\newcounter {subparagraph}[paragraph]
\renewcommand\thesection      {\@arabic\c@section}
\renewcommand\thesubsection   {\thesection.\@arabic\c@subsection}
\renewcommand\thesubsubsection{\thesubsection .\@arabic\c@subsubsection}
\renewcommand\theparagraph    {\thesubsubsection.\@arabic\c@paragraph}
\renewcommand\thesubparagraph {\theparagraph.\@arabic\c@subparagraph}
%
\def\sectcounterend{.}

\def\@seccntformat#1{\csname the#1\endcsname\sectcounterend
\hskip\betweenumberspace}

\def\@sect#1#2#3#4#5#6[#7]#8{%
  \ifnum #2>\c@secnumdepth
    \let\@svsec\@empty
  \else
    \refstepcounter{#1}%
    \protected@edef\@svsec{\@seccntformat{#1}\relax}%
  \fi
  \@tempskipa #5\relax
  \ifdim \@tempskipa>\z@
    \begingroup
      #6{%
        \@hangfrom{\hskip #3\relax\@svsec}%
          \raggedright
          \hyphenpenalty \@M%
          \interlinepenalty \@M #8\@@par}%
    \endgroup
    \csname #1mark\endcsname{#7}%
    \addcontentsline{toc}{#1}{%
      \ifnum #2>\c@secnumdepth \else
        \protect\numberline{\csname the#1\endcsname}%
      \fi
      #7}%
  \else
    \def\@svsechd{%
      #6{\hskip #3\relax
      \@svsec #8\hskip\aftertext}%
      \csname #1mark\endcsname{#7}%
      \addcontentsline{toc}{#1}{%
        \ifnum #2>\c@secnumdepth \else
          \protect\numberline{\csname the#1\endcsname}%
        \fi
        #7}}%
  \fi
  \@xsect{#5}}

%
% measures and setting of sections
%
\def\section{\@startsection{section}{1}{\z@}%
    {-16dd plus-4pt minus-4pt}{6dd}{\large\sffamily\bfseries}}
\def\subsection{\@startsection{subsection}{2}{\z@}%
    {-16dd}{6dd}{\normalsize\sffamily\itshape}}
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}%
    {-16dd}{6dd}{\normalsize\sffamily}}
\def\paragraph{\@startsection{paragraph}{4}{\z@}%
    {-16dd}{-1pt}{\normalsize\sffamily}}

\setlength\leftmargini  {\parindent}
\leftmargin  \leftmargini
\setlength\leftmarginii {\parindent}
\setlength\leftmarginiii {1.87em}
\setlength\leftmarginiv  {1.7em}
\setlength\leftmarginv  {.5em}
\setlength\leftmarginvi {.5em}
\setlength  \labelsep  {.5em}
\setlength  \labelwidth{\leftmargini}
\addtolength\labelwidth{-\labelsep}
\@beginparpenalty -\@lowpenalty
\@endparpenalty   -\@lowpenalty
\@itempenalty     -\@lowpenalty
\renewcommand\theenumi{\@arabic\c@enumi}
\renewcommand\theenumii{\@alph\c@enumii}
\renewcommand\theenumiii{\@roman\c@enumiii}
\renewcommand\theenumiv{\@Alph\c@enumiv}
\newcommand\labelenumi{\theenumi.}
\newcommand\labelenumii{(\theenumii)}
\newcommand\labelenumiii{\theenumiii.}
\newcommand\labelenumiv{\theenumiv.}
\renewcommand\p@enumii{\theenumi}
\renewcommand\p@enumiii{\theenumi(\theenumii)}
\renewcommand\p@enumiv{\p@enumiii\theenumiii}
\newcommand\labelitemi{\normalfont\bfseries --}
\newcommand\labelitemii{\normalfont\bfseries --}
\newcommand\labelitemiii{$\m@th\bullet$}
\newcommand\labelitemiv{$\m@th\cdot$}

% redefinition of the "\newtheorem" command.
%
% Usage now:
%
%     \newtheorem{env_nam}{caption}[within]{cap_font}{body_font}
% or  \newtheorem{env_nam}[numbered_like]{caption}{cap_font}{body_font}
% or  \newtheorem*{env_nam}{caption}{cap_font}{body_font}
%
% New is "cap_font" and "body_font". It stands for
% fontdefinition of the caption and the text itself.
%
% "\newtheorem*" gives a theorem without number.
%
% A defined newthoerem environment is used as described
% by Lamport.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\@thmcountersep{}
\def\@thmcounterend{.}

\def\newtheorem{\@ifstar{\@sthm}{\@Sthm}}

% definition of \newtheorem with number

\def\@Sthm#1{\@ifnextchar[{\@othm{#1}}{\@nthm{#1}}}

\def\@xnthm#1#2[#3]#4#5{\expandafter\@ifdefinable\csname #1\endcsname
   {\@definecounter{#1}\@addtoreset{#1}{#3}%
   \expandafter\xdef\csname the#1\endcsname{\expandafter\noexpand
     \csname the#3\endcsname \noexpand\@thmcountersep \@thmcounter{#1}}%
   \expandafter\xdef\csname #1name\endcsname{#2}%
   \global\@namedef{#1}{\@thm{#1}{\csname #1name\endcsname}{#4}{#5}}%
                              \global\@namedef{end#1}{\@endtheorem}}}

\def\@ynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
   {\@definecounter{#1}%
   \expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
   \expandafter\xdef\csname #1name\endcsname{#2}%
   \global\@namedef{#1}{\@thm{#1}{\csname #1name\endcsname}{#3}{#4}}%
                               \global\@namedef{end#1}{\@endtheorem}}}

\def\@othm#1[#2]#3#4#5{%
  \@ifundefined{c@#2}{\@latexerr{No theorem environment `#2'
  defined}\@eha}%
  {\expandafter\@ifdefinable\csname #1\endcsname
  {\global\@namedef{the#1}{\@nameuse{the#2}}%
  \expandafter\xdef\csname #1name\endcsname{#3}%
  \global\@namedef{#1}{\@thm{#2}{\csname #1name\endcsname}{#4}{#5}}%
  \global\@namedef{end#1}{\@endtheorem}}}}

\def\@thm#1#2#3#4{\refstepcounter
    {#1}\@ifnextchar[{\@ythm{#1}{#2}{#3}{#4}}{\@xthm{#1}{#2}{#3}{#4}}}

\def\@xthm#1#2#3#4{\@begintheorem{#2}{\csname the#1\endcsname}{#3}{#4}%
                    \ignorespaces}

\def\@ythm#1#2#3#4[#5]{\@opargbegintheorem{#2}{\csname
       the#1\endcsname}{#5}{#3}{#4}\ignorespaces}

\def\@begintheorem#1#2#3#4{\trivlist
                 \item[\hskip\labelsep{#3#1\ #2\@thmcounterend}]#4}

\def\@opargbegintheorem#1#2#3#4#5{\trivlist
      \item[\hskip\labelsep{#4#1\ #2\ (#3)\@thmcounterend}]#5}

% definition of \newtheorem* without number

\def\@sthm#1#2{\@Ynthm{#1}{#2}}

\def\@Ynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
   {\global\@namedef{#1}{\@Thm{\csname #1name\endcsname}{#3}{#4}}%
    \expandafter\xdef\csname #1name\endcsname{#2}%
    \global\@namedef{end#1}{\@endtheorem}}}

\def\@Thm#1#2#3{\@ifnextchar[{\@Ythm{#1}{#2}{#3}}{\@Xthm{#1}{#2}{#3}}}

\def\@Xthm#1#2#3{\@Begintheorem{#1}{#2}{#3}\ignorespaces}

\def\@Ythm#1#2#3[#4]{\@Opargbegintheorem{#1}
       {#4}{#2}{#3}\ignorespaces}

\def\@Begintheorem#1#2#3{#3\trivlist
                           \item[\hskip\labelsep{#2#1\@thmcounterend}]}

\def\@Opargbegintheorem#1#2#3#4{#4\trivlist
      \item[\hskip\labelsep{#3#1\ (#2)\@thmcounterend}]}

% definition of divers theorem environments

\if@envcntsect
   \def\@thmcountersep{.}
   \newtheorem{theorem}{Theorem}[section]{\bf}{\it}
\else
   \newtheorem{theorem}{Theorem}{\bf}{\it}
   \if@envcntreset
      \@addtoreset{theorem}{section}
   \else
      \@addtoreset{theorem}{chapter}
   \fi
\fi
\newtheorem*{proof}{Proof}{\it}{\rm}
\newtheorem{corollary}[theorem]{Corollary}{\bf}{\it}
\newtheorem{definition}[theorem]{Definition}{\bf}{\rm}
\newtheorem{example}[theorem]{Example}{\it}{\rm}
\newtheorem{exercise}[theorem]{Exercise}{\it}{\rm}
\newtheorem{lemma}[theorem]{Lemma}{\bf}{\it}
\newtheorem{note}[theorem]{Note}{\it}{\rm}
\newtheorem{problem}[theorem]{Problem}{\it}{\rm}
\newtheorem{proposition}[theorem]{Proposition}{\bf}{\it}
\newtheorem{question}[theorem]{Question}{\it}{\rm}
\newtheorem{remark}[theorem]{Remark}{\it}{\rm}
\newtheorem{solution}[theorem]{Solution}{\it}{\rm}

\def\@takefromreset#1#2{%
    \def\@tempa{#1}%
    \let\@tempd\@elt
    \def\@elt##1{%
        \def\@tempb{##1}%
        \ifx\@tempa\@tempb\else
            \@addtoreset{##1}{#2}%
        \fi}%
    \expandafter\expandafter\let\expandafter\@tempc\csname cl@#2\endcsname
    \expandafter\def\csname cl@#2\endcsname{}%
    \@tempc
    \let\@elt\@tempd}

\def\theopargself{\def\@opargbegintheorem##1##2##3##4##5{\trivlist
      \item[\hskip\labelsep{##4##1\ ##2\ ##3}]##5}
                  \def\@Opargbegintheorem##1##2##3##4{##4\trivlist
      \item[\hskip\labelsep{##3##1\ ##2}]}
      }

\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\qed{\ifmmode\else\unskip\quad\fi\squareforqed}
%
\newdimen\figgap\figgap=1cc
\long\def\@makesidecaption#1#2{%
   \parbox[b]{\@tempdima}{\captionstyle{\floatlegendstyle
                                         #1\floatcounterend}~#2}}
\def\sidecaption#1\caption{%
\setbox\@tempboxa=\hbox{#1\unskip}%
\if@twocolumn
 \ifdim\hsize<\textwidth\else
   \ifdim\wd\@tempboxa<\columnwidth
      \typeout{Double column float fits into single column -
            ^^Jyou'd better switch the environment. }%
   \fi
 \fi
\fi
\@tempdima=\hsize
\advance\@tempdima by-\figgap
\advance\@tempdima by-\wd\@tempboxa
\ifdim\@tempdima<3cm
    \typeout{\string\sidecaption: No sufficient room for the legend;
             using normal \string\caption. }%
   \unhbox\@tempboxa
   \let\@capcommand=\@caption
\else
   \let\@capcommand=\@sidecaption
   \leavevmode
   \unhbox\@tempboxa
   \hfill
\fi
\refstepcounter\@captype
\@dblarg{\@capcommand\@captype}}

\long\def\@sidecaption#1[#2]#3{\addcontentsline{\csname
  ext@#1\endcsname}{#1}{\protect\numberline{\csname
  the#1\endcsname}{\ignorespaces #2}}\begingroup
    \@parboxrestore
    \@makesidecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par
  \endgroup}
%
% Online material
\long\def\onlfig#1#2{\AtEndDocument{\Online\setcounter{figure}{#1}\addtocounter{figure}{-1}#2}\setcounter{figure}{#1}}
\long\def\onltab#1#2{\AtEndDocument{\Online\setcounter{table}{#1}\addtocounter{table}{-1}#2}\setcounter{table}{#1}}
\long\def\onllongtab#1#2{\AtEndDocument{\Online\setlength{\LTcapwidth}{\textwidth}\setcounter{table}{#1}%
\addtocounter{table}{-1}\onecolumn#2\twocolumn}\setcounter{table}{#1}}
\long\def\onllongtabL#1#2{\AtEndDocument{\Online\setlength{\LTcapwidth}{\textheight}\setcounter{table}{#1}%
\addtocounter{table}{-1}\onecolumn#2\twocolumn}\setcounter{table}{#1}}
\long\def\longtab#1#2{\setlength{\LTcapwidth}{\textwidth}%
\setcounter{table}{#1}\addtocounter{table}{-1}\onecolumn#2\twocolumn\setcounter{table}{#1}}
\long\def\longtabL#1#2{\setlength{\LTcapwidth}{\textheight}%
\setcounter{table}{#1}\addtocounter{table}{-1}\onecolumn#2\twocolumn\setcounter{table}{#1}}
%
% Define \acknowledgements
\def\acknowledgements{\par\addvspace{6pt}\tiny\rm
\trivlist\item[\hskip\labelsep{\em Acknowledgements.\/}]}
\def\endacknowledgements{\endtrivlist\addvspace{6pt}}
%
\newenvironment{verse}
               {\let\\\@centercr
                \list{}{\itemsep      \z@
                        \itemindent   -1.5em%
                        \listparindent\itemindent
                        \rightmargin  \leftmargin
                        \advance\leftmargin 1.5em}%
                \item\relax}
               {\endlist}
\newenvironment{quotation}
               {\list{}{\listparindent 1.5em%
                        \itemindent    \listparindent
                        \rightmargin   \leftmargin
                        \parsep        \z@ \@plus\p@}%
                \item\relax}
               {\endlist}
\newenvironment{quote}
               {\list{}{\rightmargin\leftmargin}%
                \item\relax}
               {\endlist}
\if@compatibility
\newenvironment{titlepage}
    {%
      \if@twocolumn
        \@restonecoltrue\onecolumn
      \else
        \@restonecolfalse\newpage
      \fi
      \thispagestyle{empty}%
      \setcounter{page}\z@
    }%
    {\if@restonecol\twocolumn \else \newpage \fi
    }
\else
\newenvironment{titlepage}
    {%
      \if@twocolumn
        \@restonecoltrue\onecolumn
      \else
        \@restonecolfalse\newpage
      \fi
      \thispagestyle{empty}%
      \setcounter{page}\@ne
    }%
    {\if@restonecol\twocolumn \else \newpage \fi
     \if@twoside\else
        \setcounter{page}\@ne
     \fi
    }
\fi
% Appendix
\newcounter{append}
\setcounter{append}{0}
\newenvironment{appendix}{\par
\def\@hangfrom##1{\setbox\@tempboxa\hbox{{##1}}%
      \hangindent \parindent\noindent\box\@tempboxa}
\def\@seccntformat##1{\csname theap##1\endcsname\hskip\betweenumberspace}
  \setcounter{section}{\value{append}}%
  \setcounter{subsection}{0}%
  \setcounter{figure}{0}%
  \setcounter{table}{0}%
  \newcommand\theapsection{Appendix \@Alph\c@section:}%
  \newcommand\theapsubsection{\@Alph\c@section.\@arabic\c@subsection.}%
  \newcommand\theapsubsubsection{\theapsubsection\@arabic\c@subsubsection.}%
  \renewcommand\thesection{\@Alph\c@section}%
  \renewcommand\thesubsection{\@Alph\c@section.\@arabic\c@subsection}%
  \renewcommand\thesubsubsection{\thesubsection.\@arabic\c@subsubsection}%
  \renewcommand\theequation{\@Alph\c@section.\@arabic\c@equation}%
  \renewcommand\thefigure{\@Alph\c@section.\@arabic\c@figure}%
  \renewcommand\thetable{\@Alph\c@section.\@arabic\c@table}%
  \@addtoreset{equation}{section}%
  \@addtoreset{figure}{section}%
  \@addtoreset{table}{section}%
  \def\subfigures{\stepcounter{figure}\setcounter{auth}{\value{figure}}%
  \setcounter{figure}{0}%
  \def\thefigure{\@Alph\c@section\@arabic\c@auth\alph{figure}}%
  \def\resetsubfig{\setcounter{figure}{\value{auth}}}}}
{
  \setcounter{section}{0}%
  \setcounter{subsection}{0}%
  \setcounter{figure}{0}%
  \setcounter{table}{0}%
  \renewcommand\thesection{\c@section}%
  \renewcommand\thesubsection{\@arabic\c@subsection}%
  \renewcommand\thesubsubsection{\@arabic\c@subsubsection}%
  \renewcommand\theequation{\@arabic\c@equation}%
  \renewcommand\thefigure{\@arabic\c@figure}%
  \renewcommand\thetable{\@arabic\c@table}%
  \addtocounter{append}{1}
}
%
\setlength\arraycolsep{2.5\p@}
\setlength\tabcolsep{6\p@}
\setlength\arrayrulewidth{.4\p@}
\setlength\doublerulesep{2\p@}
\setlength\tabbingsep{\labelsep}
\skip\@mpfootins = \skip\footins
\setlength\fboxsep{3\p@}
\setlength\fboxrule{.4\p@}
\renewcommand\theequation{\@arabic\c@equation}
\newcounter{figure}
\renewcommand\thefigure{\@arabic\c@figure}
\def\fps@figure{tbp}
\def\ftype@figure{1}
\def\ext@figure{lof}
\def\fnum@figure{\figurename\,\thefigure}
\newenvironment{figure}
               {\@float{figure}}
               {\resetsubfig\end@float}
\newenvironment{figure*}
               {\@dblfloat{figure}}
               {\resetsubfig\end@dblfloat}
\let\resetsubfig\relax
\def\subfigures{\stepcounter{figure}\setcounter{auth}{\value{figure}}%
\setcounter{figure}{0}\def\thefigure{\@arabic\c@auth\alph{figure}}%
\def\resetsubfig{\setcounter{figure}{\value{auth}}}}
\newcounter{table}
\renewcommand\thetable{\@arabic\c@table}
\def\fps@table{tbp}
\def\ftype@table{2}
\def\ext@table{lot}
\def\fnum@table{\tablename~\thetable}
\newenvironment{table}
               {\small\@float{table}}
               {\end@float}
\newenvironment{table*}
               {\small\@dblfloat{table}}
               {\end@dblfloat}

\def \@floatboxreset {%
        \reset@font
        \small
        \@setnobreak
        \@setminipage
}

\newlength\abovecaptionskip
\newlength\belowcaptionskip
\setlength\abovecaptionskip{10\p@}
\setlength\belowcaptionskip{0\p@}
\newcommand\leftlegendglue{}

\def\fig@type{figure}

\newdimen\figcapgap\figcapgap=5pt
\newdimen\tabcapgap\tabcapgap=10pt

\@ifundefined{floatlegendstyle}{\def\floatlegendstyle{\bf}}{}
\def\floatcounterend{.}

\long\def\@caption#1[#2]#3{\par\addcontentsline{\csname
  ext@#1\endcsname}{#1}{\protect\numberline{\csname
  the#1\endcsname}{\ignorespaces #2}}\begingroup
    \@parboxrestore
    \@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par
  \endgroup}

\def\capstrut{\vrule\@width\z@\@height\topskip}
\@ifundefined{captionstyle}{\def\captionstyle{\normalfont\small}}{}

\long\def\@makecaption#1#2{%
 \ifx\@captype\fig@type
   \vskip\figcapgap
   \setbox\@tempboxa\hbox{{\floatlegendstyle #1\floatcounterend}
   \capstrut #2}%
   \ifdim \wd\@tempboxa >\hsize
     {\floatlegendstyle #1\floatcounterend} \capstrut #2\par
   \else
     \hbox to\hsize{\leftlegendglue\unhbox\@tempboxa\hfil}%
   \fi
 \else
   {\floatlegendstyle #1\floatcounterend} \capstrut #2\par
   \vskip\tabcapgap
 \fi}
% Define `acknowledgement' environment
\def\acknowledgement{\par\addvspace{17pt}\tiny\rm
\trivlist\item[\hskip\labelsep
{\it\ackname}]}
\def\endacknowledgement{\endtrivlist\addvspace{6pt}}
% Define `noteadd' environment
\def\noteadd{\par\addvspace{17pt}\small\rm
\trivlist\item[\hskip\labelsep
{\it\noteaddname}]}
\def\endnoteadd{\endtrivlist\addvspace{6pt}}

\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}
\DeclareRobustCommand*\cal{\@fontswitch\relax\mathcal}
\DeclareRobustCommand*\mit{\@fontswitch\relax\mathnormal}
\newcommand\@pnumwidth{1.55em}
\newcommand\@tocrmarg{2.55em}
\newcommand\@dotsep{4.5}
\setcounter{tocdepth}{3}
\newcommand\tableofcontents{%
    \section*{\contentsname
        \@mkboth{%
           \MakeUppercase\contentsname}{\MakeUppercase\contentsname}}%
    \@starttoc{toc}%
    }
\newcommand*\l@part[2]{%
  \ifnum \c@tocdepth >-2\relax
    \addpenalty\@secpenalty
    \addvspace{2.25em \@plus\p@}%
    \begingroup
      \setlength\@tempdima{3em}%
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      {\leavevmode
       \large \bfseries #1\hfil \hb@xt@\@pnumwidth{\hss #2}}\par
       \nobreak
       \if@compatibility
         \global\@nobreaktrue
         \everypar{\global\@nobreakfalse\everypar{}}%
      \fi
    \endgroup
  \fi}
\newcommand*\l@section[2]{%
  \ifnum \c@tocdepth >\z@
    \addpenalty\@secpenalty
    \addvspace{1.0em \@plus\p@}%
    \setlength\@tempdima{1.5em}%
    \begingroup
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      \leavevmode \bfseries
      \advance\leftskip\@tempdima
      \hskip -\leftskip
      #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\par
    \endgroup
  \fi}
\newcommand*\l@subsection{\@dottedtocline{2}{1.5em}{2.3em}}
\newcommand*\l@subsubsection{\@dottedtocline{3}{3.8em}{3.2em}}
\newcommand*\l@paragraph{\@dottedtocline{4}{7.0em}{4.1em}}
\newcommand*\l@subparagraph{\@dottedtocline{5}{10em}{5em}}
\newcommand\listoffigures{%
    \section*{\listfigurename
      \@mkboth{\MakeUppercase\listfigurename}%
              {\MakeUppercase\listfigurename}}%
    \@starttoc{lof}%
    }
\newcommand*\l@figure{\@dottedtocline{1}{1.5em}{2.3em}}
\newcommand\listoftables{%
    \section*{\listtablename
      \@mkboth{%
          \MakeUppercase\listtablename}{\MakeUppercase\listtablename}}%
    \@starttoc{lot}%
    }
\let\l@table\l@figure
\newdimen\bibindent
\setlength\bibindent{\parindent}
\def\@biblabel#1{}
\def\@cite#1#2{{#1\if@tempswa , #2\fi}}
\newenvironment{thebibliography}[1]
     {\begingroup\section*{{\normalsize\refname}
        \@mkboth{\refname}{\refname}}\tiny
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
           \leftmargin\bibindent
           \setlength{\itemindent}{-\leftmargin}
           \@openbib@code
           \usecounter{enumiv}%
           \let\p@enumiv\@empty
           \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy\clubpenalty4000\widowpenalty4000%
      \sfcode`\.\@m}
     {\endlist\par\endgroup\if@longauth\kern6pt\hrule\kern6pt\institutename\@longauthfalse\fi
      \def\@noitemerr{\@latex@warning{Empty `thebibliography' environment}}}%


\newcommand\newblock{\hskip .11em\@plus.33em\@minus.07em}
\let\@openbib@code\@empty
\newenvironment{theindex}
               {\if@twocolumn
                  \@restonecolfalse
                \else
                  \@restonecoltrue
                \fi
                \columnseprule \z@
                \columnsep 35\p@
                \twocolumn[\section*{\indexname}]%
                \@mkboth{\MakeUppercase\indexname}%
                        {\MakeUppercase\indexname}%
                \thispagestyle{plain}\parindent\z@
                \parskip\z@ \@plus .3\p@\relax
                \let\item\@idxitem}
               {\if@restonecol\onecolumn\else\clearpage\fi}
\newcommand\@idxitem{\par\hangindent 40\p@}
\newcommand\subitem{\@idxitem \hspace*{20\p@}}
\newcommand\subsubitem{\@idxitem \hspace*{30\p@}}
\newcommand\indexspace{\par \vskip 10\p@ \@plus5\p@ \@minus3\p@\relax}
\renewcommand\footnoterule{%
  \kern-3\p@
  \hrule\@width.4\columnwidth
  \kern2.6\p@}
\newcommand\@makefntext[1]{%
    \noindent
    \hb@xt@\bibindent{\hss\@makefnmark\enspace}#1}
%
\newcommand\listofobjects{\if@nyobjects
  \IfFileExists{\jobname.obj}%
               {\section*{\listobjectname}%
                \@starttoc{obj}}%
               {\begingroup
                   \makeatletter
                   \if@filesw
                      \newwrite\tf@obj
                      \immediate\openout\tf@obj\jobname.obj
                      \relax
                   \fi
                   \global\@nobreakfalse
                \endgroup}\fi
               }
%
\newcommand*\l@obj[2]{\noindent`#1' on page #2\par}
%
\DeclareRobustCommand{\object}[1]{#1\global\let\if@nyobjects\iftrue
\addcontentsline{obj}{obj}{#1}}
%
\newcommand\contentsname{Contents}
\newcommand\listfigurename{List of Figures}
\newcommand\listobjectname{List of Objects}
\newcommand\listtablename{List of Tables}
\newcommand\refname{References}
\newcommand\indexname{Index}
\newcommand\figurename{Fig.}
\newcommand\tablename{Table}
\newcommand\partname{Part}
\newcommand\appendixname{Appendix}
\newcommand\abstractname{ABSTRACT}
\newcommand\rnotename{(Research Note)}
\newcommand\rnotname{(RN)}
\newcommand\lettername{\textsc{Letter to the Editor}}
\newcommand\ackname{Acknowledgements.}
\newcommand\noteaddname{Note added in proof}
\newcommand\today{}
\edef\today{\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\day, \number\year}
\setlength\columnsep{12pt}
\setlength\columnseprule{0\p@}
\frenchspacing
\clubpenalty=10000
\widowpenalty=10000
\def\thisbottomragged{\def\@textbottom{\vskip\z@ plus.0001fil
\global\let\@textbottom\relax}}
\pagestyle{headings}
\pagenumbering{arabic}
\if@referee
  \setlength{\textwidth}{0.75\textwidth}
  \def\baselinestretch{1.5}
  \let\AALogo\relax
  \onecolumn
  \AtEndDocument{\listofobjects}
\else
\if@onecolumn
\onecolumn
\else
  \twocolumn
\fi\fi
\sloppy
\flushbottom
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\sq{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\squareforqed
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

\def\sun{\hbox{$\odot$}}
\def\la{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\sim\cr}}}}}
\def\ga{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\sim\cr}}}}}
\def\degr{\hbox{$^\circ$}}
\def\arcmin{\hbox{$^\prime$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\utw{\smash{\rlap{\lower5pt\hbox{$\sim$}}}}
\def\udtw{\smash{\rlap{\lower6pt\hbox{$\approx$}}}}
\def\fd{\hbox{$.\!\!^{\rm d}$}}
\def\fh{\hbox{$.\!\!^{\rm h}$}}
\def\fm{\hbox{$.\!\!^{\rm m}$}}
\def\fs{\hbox{$.\!\!^{\rm s}$}}
\def\fdg{\hbox{$.\!\!^\circ$}}
\def\farcm{\hbox{$.\mkern-4mu^\prime$}}
\def\farcs{\hbox{$.\!\!^{\prime\prime}$}}
\def\fp{\hbox{$.\!\!^{\scriptscriptstyle\rm p}$}}
\def\cor{\mathrel{\mathchoice {\hbox{$\widehat=$}}{\hbox{$\widehat=$}}
{\hbox{$\scriptstyle\hat=$}}
{\hbox{$\scriptscriptstyle\hat=$}}}}
\def\sol{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr\sim\cr<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\sim\cr
<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr\sim\cr
<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\sim\cr<\cr}}}}}
\def\sog{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr\sim\cr>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\sim\cr
>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
\sim\cr>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\sim\cr>\cr}}}}}
\def\lse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\simeq\cr}}}}}
\def\gse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\simeq\cr}}}}}
\def\grole{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\noalign{\vskip-1pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\noalign{\vskip-0.5pt}<\cr}}}}}
\def\leogr{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\noalign{\vskip-1pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\noalign{\vskip-0.5pt}>\cr}}}}}
\def\loa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\approx\cr}}}}}
\def\goa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\approx\cr}}}}}
\def\diameter{{\ifmmode\mathchoice
{\ooalign{\hfil\hbox{$\displaystyle/$}\hfil\crcr
{\hbox{$\displaystyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\textstyle/$}\hfil\crcr
{\hbox{$\textstyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\scriptstyle/$}\hfil\crcr
{\hbox{$\scriptstyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\scriptscriptstyle/$}\hfil\crcr
{\hbox{$\scriptscriptstyle\mathchar"20D$}}}}
\else{\ooalign{\hfil/\hfil\crcr\mathhexbox20D}}%
\fi}}

\def\getsto{\mathrel{\mathchoice {\vcenter{\offinterlineskip
\halign{\hfil
$\displaystyle##$\hfil\cr\gets\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\gets\cr\to\cr}}}}}
\def\lid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr<\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr<\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr
\noalign{\vskip0.9pt}=\cr}}}}}
\def\gid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr>\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr>\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr
\noalign{\vskip0.9pt}=\cr}}}}}
\def\bbbr{{\rm I\!R}} %reelle Zahlen
\def\bbbm{{\rm I\!M}}
\def\bbbn{{\rm I\!N}} %natuerliche Zahlen
\def\bbbf{{\rm I\!F}}
\def\bbbh{{\rm I\!H}}
\def\bbbk{{\rm I\!K}}
\def\bbbp{{\rm I\!P}}
\def\bbbone{{\mathchoice {\rm 1\mskip-4mu l} {\rm 1\mskip-4mu l}
{\rm 1\mskip-4.5mu l} {\rm 1\mskip-5mu l}}}
\def\bbbc{{\mathchoice {\setbox0=\hbox{$\displaystyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}}}
\def\bbbq{{\mathchoice {\setbox0=\hbox{$\displaystyle\rm
Q$}\hbox{\raise
0.05\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle\rm Q$}\hbox{\raise
0.05\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle\rm Q$}\hbox{\raise
0.05\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.8\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm Q$}\hbox{\raise
0.05\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.8\ht0\hss}\box0}}}}
\def\bbbt{{\mathchoice {\setbox0=\hbox{$\displaystyle\rm
T$}\hbox{\hbox to0pt{\kern0.25\wd0\vrule height0.95\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle\rm T$}\hbox{\hbox
to0pt{\kern0.25\wd0\vrule height0.95\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle\rm T$}\hbox{\hbox
to0pt{\kern0.25\wd0\vrule height0.95\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm T$}\hbox{\hbox
to0pt{\kern0.25\wd0\vrule height0.95\ht0\hss}\box0}}}}
\def\bbbs{{\mathchoice
{\setbox0=\hbox{$\displaystyle\rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.38\wd0\vrule height0.45\ht0\hss}\hbox
to0pt{\kern0.52\wd0\vrule height0.5\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle \rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.38\wd0\vrule height0.45\ht0\hss}\hbox
to0pt{\kern0.52\wd0\vrule height0.5\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle \rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.38\wd0\vrule height0.45\ht0\hss}\raise0.05\ht0\hbox
to0pt{\kern0.52\wd0\vrule height0.45\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.38\wd0\vrule height0.45\ht0\hss}\raise0.05\ht0\hbox
to0pt{\kern0.52\wd0\vrule height0.45\ht0\hss}\box0}}}}
\def\bbbz{{\mathchoice {\hbox{$\sf\textstyle Z\kern-0.4em Z$}}
{\hbox{$\sf\textstyle Z\kern-0.4em Z$}}
{\hbox{$\sf\scriptstyle Z\kern-0.3em Z$}}
{\hbox{$\sf\scriptscriptstyle Z\kern-0.2em Z$}}}}
\def\ts{\thinspace}
%
% Bibliography and bibfile
\def\aj{AJ}%
          % Astronomical Journal
\def\actaa{Acta Astron.}%
          % Acta Astronomica
\def\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
          % Astrophysical Journal
\def\apjl{ApJ}%
          % Astrophysical Journal, Letters
\def\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}%
          % Applied Optics
\def\apss{Ap\&SS}%
          % Astrophysics and Space Science
\def\aap{A\&A}%
          % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
          % Astronomicheskii Zhurnal
\def\baas{BAAS}%
          % Bulletin of the AAS
\def\bac{Bull. astr. Inst. Czechosl.}%
          % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{Chinese Astron. Astrophys.}%
          % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J. Astron. Astrophys.}%
          % Chinese Journal of Astronomy and Astrophysics
\def\icarus{Icarus}%
          % Icarus
\def\jcap{J. Cosmology Astropart. Phys.}%
          % Journal of Cosmology and Astroparticle Physics
\def\jrasc{JRASC}%
          % Journal of the RAS of Canada
\def\mnras{MNRAS}%
          % Monthly Notices of the RAS
\def\memras{MmRAS}%
          % Memoirs of the RAS
\def\na{New A}%
          % New Astronomy
\def\nar{New A Rev.}%
          % New Astronomy Review
\def\pasa{PASA}%
          % Publications of the Astron. Soc. of Australia
\def\pra{Phys.~Rev.~A}%
          % Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}%
          % Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}%
          % Physical Review C
\def\prd{Phys.~Rev.~D}%
          % Physical Review D
\def\pre{Phys.~Rev.~E}%
          % Physical Review E
\def\prl{Phys.~Rev.~Lett.}%
          % Physical Review Letters
\def\pasp{PASP}%
          % Publications of the ASP
\def\pasj{PASJ}%
          % Publications of the ASJ
\def\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%
          % Revista Mexicana de Astronomia y Astrofisica
\def\skytel{S\&T}%
          % Sky and Telescope
\def\solphys{Sol.~Phys.}%
          % Solar Physics
\def\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\def\ssr{Space~Sci.~Rev.}%
          % Space Science Reviews
\def\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
          % Nature
\def\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\def\aplett{Astrophys.~Lett.}%
          % Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\def\jgr{J.~Geophys.~Res.}%
          % Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.~Phys.~A}%
          % Nuclear Physics A
\def\physrep{Phys.~Rep.}%
          % Physics Reports
\def\physscr{Phys.~Scr}%
          % Physica Scripta
\def\planss{Planet.~Space~Sci.}%
          % Planetary Space Science
\def\procspie{Proc.~SPIE}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
%
\uchyph=0
% 
\long\def\Online{\if@online\else\@onlinetrue
\clearpage
\def\ps@Onlheadings{%
    \let\@oddfoot\@empty\let\@evenfoot\@empty
    \def\@evenhead{\hfil\leftmark, {\it Online Material p~\thepage}\hfil}%
    \def\@oddhead{\hfil\rightmark, {\it Online Material p~\thepage}\hfil}%
    \let\@mkboth\@gobbletwo
    \let\sectionmark\@gobble
    \let\subsectionmark\@gobble
    }
\setcounter{page}{1}
\pagestyle{Onlheadings}
%% 2008
%% \twocolumn[\vspace*{4cm}\noindent{\sffamily\bfseries\Huge\centerline{Online Material}}]
%% \vfill
%% \clearpage
\fi}
\AtBeginDocument{\@ifpackageloaded{natbib}{\let\bibpreamble\relax\newcommand{\bibfont}{\tiny}%
\renewenvironment{thebibliography}[1]{%
 \bibsection\parindent \z@\bibpreamble\bibfont\list
   {\@biblabel{\arabic{NAT@ctr}}}{\@bibsetup{#1}%
    \setcounter{NAT@ctr}{0}}%
    \ifNAT@openbib
      \renewcommand\newblock{\par}
    \else
      \renewcommand\newblock{\hskip .11em \@plus.33em \@minus.07em}%
    \fi
    \sloppy\clubpenalty4000\widowpenalty4000
    \sfcode`\.=1000\relax
    \let\citeN\cite \let\shortcite\cite
    \let\citeasnoun\cite
 }{\if@longauth\kern6pt\hrule\kern6pt\institutename\@longauthfalse\fi\def\@noitemerr{%
  \PackageWarning{natbib}
     {Empty `thebibliography' environment}}%
  \endlist\vskip-\lastskip}}{}
\@ifpackageloaded{longtable}{%
\def\LT@makecaption#1#2#3{%
  \LT@mcol\LT@cols c{\hbox to\z@{\hss\parbox[t]\LTcapwidth{%
    \small\sbox\@tempboxa{#1{{\bfseries#2.} }#3}%
    \ifdim\wd\@tempboxa>\hsize
      #1{{\bfseries#2.} }#3%
    \else
      \hbox to\hsize{\box\@tempboxa\hfil}%
    \fi
    \endgraf\vskip\baselineskip}%
  \hss}}}}{}
}%AtBeginDocument
%
\endinput
%%
%% End of file `aa.cls'.

